Distributed Instruments for Planetary Surface Science: Scientific Opportunities and Technology Feasibility

In this paper, we assess the scientific promise and technology feasibility of distributed instruments for planetary science. A distributed instrument is an instrument designed to collect spatially and temporally correlated data from multiple networked, geographically distributed point sensors. Distributed instruments are ubiquitous in Earth science, where they are routinely employed for weather and climate science, seismic studies and resource prospecting, and detection of industrial emissions. However, to date, their adoption in planetary surface science has been minimal. It is natural to ask whether this lack of adoption is driven by low potential to address high-priority questions in planetary science; immature technology; or both. To address this question, we survey high-priority planetary science questions that are uniquely well-suited to distributed instruments. We identify four areas of research where distributed instruments hold promise to unlock answers that are largely inaccessible to monolithic sensors, namely, weather and climate studies of Mars; localization of seismic events on rocky and icy bodies; localization of trace gas emissions, primarily on Mars; and magnetometry studies of internal composition. Next, we survey enabling technologies for distributed sensors and assess their maturity. We identify sensor placement (including descent and landing on planetary surfaces), power, and instrument autonomy as three key areas requiring further investment to enable future distributed instruments. Overall, this work shows that distributed instruments hold great promise for planetary science, and paves the way for follow-on studies of future distributed instruments for Solar System in-situ science.

==> authors.tex <==
\section{Biography of Authors}

\begin{multicols}{2}
\begin{wrapfigure}{r}{0.15\textwidth}
    \centering
    \vspace{-.1cm}
    \includegraphics[width=0.145\textwidth]{bio/FedericoRossi}
\end{wrapfigure}

\textbf{Dr. Federico Rossi} is a Robotics Technologist with the Maritime and Multi-Agent Autonomy Group at the Jet Propulsion Laboratory, California Institute of Technology.
He earned a Ph.D. in Aeronautics and Astronautics from Stanford University in 2018, a M.Sc. in Space Engineering from Politecnico di Milano and the Diploma from the Alta Scuola Politecnica in 2013.
Federico's research focuses on optimal control and distributed decision-making in multi-agent robotic systems, with applications to planetary exploration and Earth science.

\begin{wrapfigure}{r}{0.15\textwidth}
	\centering
	\vspace{-.45cm}
	\includegraphics[width=0.145\textwidth]{bio/BobAnderson}
\end{wrapfigure}

\textbf{Dr. Robert C. Anderson} 
 is a senior member of the Geophysics and Planetary Geosciences group at the Jet Propulsion Laboratory (JPL).
 Dr. Anderson received his B.Sc. and M.Sc. in Geology from Old Dominion University in 1979 and 1985, respectively. 
In 1995, he received a Doctor of Philosophy from the University of Pittsburgh in geology with an emphasis on visible and near infrared remote sensing.
 Dr. Anderson worked on the Mars Pathfinder Project as science support for the Mineralogy and Geochemistry Science Operations Group, and he was the Investigation Scientist for the Rock Abrasion Tool (RAT) and science support for Mission Operations on the Mars Exploration Rover (MER) mission. Currently, Dr. Anderson is an Investigation Scientist for the Mars Science Laboratory (MSL) Sample Acquisition / Sample Handling (SA/SPaH) subsystem.


\begin{wrapfigure}{r}{0.15\textwidth}
    \centering
    \vspace{-.45cm}
    \includegraphics[width=0.145\textwidth]{bio/Saptarshi}
    \vspace{-2em}
\end{wrapfigure}
\textbf{Dr. Saptarshi Bandyopadhyay} is a Robotics Technologist at the Jet Propulsion Laboratory, California Institute of Technology. 
He received his Ph.D. in Aerospace Engineering in January 2016 from the University of Illinois at Urbana-Champaign (UIUC). 
He received his Dual Degree (B.Tech and M.Tech) in Aerospace Engineering in 2010 from the Indian Institute of Technology Bombay, India. 
Saptarshi's research interests include aerospace systems, robotics, multi-agent systems and swarms, dynamics and controls, estimation theory, probability theory, and systems engineering. 

\begin{wrapfigure}{r}{0.15\textwidth}
	\centering
	\vspace{-.45cm}
	\includegraphics[width=0.145\textwidth]{bio/ErikBrandon}
\end{wrapfigure}

\textbf{Dr. Erik J. Brandon} is currently the Chief Technologist for the Power and Sensor Systems Section at the Jet Propulsion Laboratory (JPL) in Pasadena, CA. Prior to this role, he served for nine years as the Technical Group Supervisor for the Electrochemical Technologies Group at JPL. His research interests include the design of advanced integrated passive components and energy storage technologies for small spacecraft power sources, flexible electronics and multi-functional materials for deployable space structures, advanced thermoelectric devices for power generation, primary batteries for deep space missions and supercapacitors and supercapacitor/hybrid battery technologies for extreme environment applications. He is currently leading the development of batteries for the Europa Lander Pre-Project, as well as a chemical heat integrated power system technology demonstration for extreme environment survival. Dr. Brandon also serves as a reviewer or external advisor for several Department of Energy and NASA programs. He received the Ph.D. degree in Inorganic Chemistry from the University of Utah. 

\begin{wrapfigure}{r}{0.15\textwidth}
	\centering
	\vspace{-.45cm}
        \includegraphics[width=0.145\textwidth]{bio/AshishGoel_s}
\end{wrapfigure}


\textbf{Dr. Ashish Goel} 
 is a Research Technologist at the Jet Propulsion Laboratory in the Robotic Surface Mobility group. Ashish received his M.Sc. and Ph.D. in Aeronautics and Astronautics from Stanford University, and his Bachelors degree in Engineering Physics from Indian Institute of Technology Bombay, India. Prior to joining JPL, Ashish also worked as a postdoctoral researcher in the Graduate Aerospace Laboratories at Caltech. In addition to robotic mobility systems, his research interests include embedded systems, physics-based modeling, mission design, smallsats and CubeSats, precision GNSS and high-altitude ballooning. 


\begin{wrapfigure}{r}{0.15\textwidth}
    \centering
    \vspace{-.45cm}
    \includegraphics[width=0.145\textwidth]{bio/josh}
\end{wrapfigure}

\textbf{Dr. Joshua Vander Hook} 
is the Technical Group Supervisor of the AI, Observation Planning and Analysis
Group at the Jet Propulsion Laboratory, California Institute of Technology.
He leads distributed system design for a few NASA and
Department of Defense tasks and contributes as much as possible to a few more.
His Ph.D. work focused on designing and deploying a cooperative mobile sensor
network for locating invasive species.  He has two robotic systems
patents, and is mostly interested in optimal experiment design, cooperative
Bayesian games, and the design of multi-agent systems.  


\begin{wrapfigure}{r}{0.15\textwidth}
	\centering
	\vspace{-.45cm}
	\includegraphics[width=0.145\textwidth]{bio/MichaelMischna}
\end{wrapfigure}

\textbf{Dr. Michael Mischna} is a research scientist at the Jet Propulsion Laboratory, and Principal Scientist of the Mars Exploration Program Office.  Previously, he was supervisor of the Planetary and Exoplanetary Atmospheres group, and Deputy Chief Scientist of JPL’s Planetary Science Directorate.  He received a Ph.D. and M.S. in Geophysics and Space Physics in 2004 from UCLA, an M.S. in Meteorology from The Pennsylvania State University in 1999 and a B.S. with Honors in Atmospheric Science from Cornell University in 1997.  His research interests lie in the climate and atmospheres of terrestrial planets, with an emphasis on long-term climate change and atmospheric evolution.

\vfill\null
\columnbreak

\begin{wrapfigure}{r}{0.15\textwidth}
	\centering
	\vspace{-.45cm}
	\includegraphics[width=0.145\textwidth]{bio/MickeyVillarreal}
\end{wrapfigure}

\textbf{Dr. Michaela Villarreal} is a planetary scientist at the Jet Propulsion Laboratory, California Institute of Technology.  She received her M.S. and Ph.D. in Space Physics and Geophysics from UCLA in 2016 and 2018, respectively, and her Bachelor’s degree in Planetary Science from UC Berkeley in 2011. Michaela’s research focuses on the solar wind and plasma interactions with planetary bodies as well as electromagnetic sounding of solid bodies.

\begin{wrapfigure}{r}{0.15\textwidth}
	\centering
	\vspace{-.45cm}
	\includegraphics[width=0.145\textwidth]{bio/MarkWronkiewicz}
\end{wrapfigure}

\textbf{Dr. Mark Wronkiewicz} 
is a Data Scientist at the Jet Propulsion Laboratory, California
Institute of Technology working in the Machine Learning and Instrument Autonomy 
(MLIA) group. He currently leads a team building autonomy software to detect and
characterize cell-sized life for the broader Ocean Worlds Life Surveyor (OWLS) 
project. More broadly, he is interested in using machine learning and autonomy
to advance robotic and crewed exploration of the solar system. Mark earned his 
PhD in Neuroscience and B.Sc. in Biomedical Engineering.

\end{multicols}


==> pathfinders_and_missions.tex <==
\section{Instrument Concepts and Pathfinders}
\label{ch:pathfinders}

\frtodo{Can we merge Sections \ref{ch:sciencecase} and \ref{ch:pathfinders}??}

\revmm{In this section, we explore in detail the scientific promise of a distributed instrument for each of the four topics identified in Section \ref{ch:sciencecase}; for each topic, we also draft and a notional distributed instrument architecture, recognize key challenges and weaknesses of the proposed architecture, and identify a high-level strategy to overcome these challenges. The end of this section presents a discussion of two challenges that are common to all architecture, namely, cost and survivability.}

\input{science/seismography}
\input{science/magnetometry}
\input{science/trace_gas}
\input{science/mars_atmosphere}

\subsection{Common challenges}
\label{sec:sciencecase:common-challenges}

\revmm{We conclude this chapter by discussing two challenges that broadly affect all outlined concepts: cost and survivability.

\subparagraph{Cost} For many distributed instruments, basic sensor costs do not present a significant hurdle, nor do they offer technology development challenges; rather, there remain unresolved challenges concerning methods of deployment—how the sensor payloads are to be carried and deployed across the planet — and the carrier system by which the sensors are delivered. 
Despite the small nature of each individual sensor, costs associated with a ‘‘mothership’’ or payload carrier may increase mission costs for a dedicated mission. These concerns are especially relevant for instruments that require global distribution, e.g., those targeted to climate and magnetometry investigations. The requirement to deploy across a range of latitudes and longitudes presents non-trivial questions about how the sensors are to be released—whether during approach to the body of interest, or by an orbiting carrier.  This uncertainty requires additional analysis, and the best solution may present additional costs to a notional stand-alone mission design.  An alternative approach, deployment as a series of secondary, ‘‘ride-along’’ SmallSat payloads, also requires further study.
For Mars instruments, outside studies of landing systems such as the Small High Impact Energy Landing Device (SHIELD) \citep{Ref:Barba2019_SHIELD} have assessed the survivability of many elements similar to the notional payloads discussed in this chapter, and found the basic payload elements could survive a hard landing —- this provides one means by which to deploy individual components of the distributed payload.  Softer landing systems (e.g., Mars\textsubscript{DROP} \citep{MarsDrop}) are reasonable alternatives as well.  Both approaches, however, are not yet sufficiently mature for flight, and require additional development and cost assessment for use with multiple individual deployments.



\paragraph{Survivability} Individual elements, with low SWaP, must also manage potentially challenging environmental conditions, and it is also necessary to ensure a sufficiently long lifetime for each sensor package.  
For all the science concepts of interest, multi-year investigations are highly desirable to maximize the likelihood of detecting events of interest and to capture seasonal variability.
For instance, a strawman threshold mission investigating the Martian climate would last a minimum of one Mars year, so as to cover a full year of the three primary Martian climate cycles.  Ideally, though, a mission lifetime of several Mars years is more desirable so as to capture as much of the interannual variability in the climate cycles as possible (while CO$_2$ and water cycles are mostly consistent year over year, the dust cycle is highly variable and unpredictable; e.g., \citep{zurek1993interannual}).
Likewise, a mission to investigate seismic activity should perform monitoring over a long time horizon; for reference, InSight's reference mission was baselined to last one Martian year (corresponging to approximately two Earth years); at the time of writing, the mission has been extended by an additional Martian year.
Similarly, a distributed instrument designed to observe and localize trace gas plumes should last months to years, so as to increase the likelihood of observing and, critically, localizing a meaningful number of plumes.
Survivability concerns are especially critical for instruments requiring global coverage, e.g., climate investigations.
High latitude (polar) elements of the distributed instrument may experience extended periods of low temperature and darkness throughout the polar winter.  This can, in part, be mitigated by deployment of sensors only to mid- or low latitudes, but to enable true global coverage, it is necessary to deploy elements to polar latitudes, and therefore to keep elements of these higher latitude payloads and their electronics warm and energized.  This will impact payload design and SWaP of the payload.
}


==> summary.tex <==
\section{Executive Summary}

The goal of this study is to assess the science promise and technology feasibility of \emph{distributed instruments}. 

A distributed instrument is an instrument designed to collect spatially and temporally correlated data from many networked, geographically distributed point sensors.
A distributed instrument is more than the sum of its sensors: by strategically scheduling measurements across a region to capture data with spatial context, it can provide insight into spatially and temporally correlated phenomena that is impossible to obtain using only rovers or orbiters.

It is generally recognized that distributed instruments hold promise to unlock answers to key questions in planetary science that cannot be addressed by point measurements or orbiters alone, including how solar tides influence the  atmospheres of bodies like Mars, Venus, and Titan, how pressure waves propagate across a planet, the surface locations from where trace gas emissions originate, and what the interior composition of icy bodies is \citep{Beaty2012MEPAG,BanfieldEtAl2020MEPAG,Barba2019ICESAG}.

Despite this, very few distributed instrument designs have emerged at JPL. The goal of this project is to bridge this gap by:

\begin{itemize}
\item	Identifying and ranking high-priority scientific questions that can be uniquely addressed by distributed instruments with existing or tipping-point technologies;
\item	Identifying and ranking technologies that should be further developed to ensure the technology feasibility and to maximize the scientific returns of promising distributed instruments;
\item	Identifying programmatic steps that should be taken to foster the design, development, and deployment of distributed instruments at JPL. 
\end{itemize}

To address these questions, we consulted thirty-four scientists and technologists at JPL and in the wider NASA community. These are our findings.

\paragraph{High-Priority Science Questions}

\begin{displayquote}
\emph{Distributed instruments are uniquely well positioned to address a number of high priority scientific questions.}
\end{displayquote}

Our findings unequivocally show that distributed instruments hold unique promise to address high-priority questions that cannot be addressed with either remote sensing from orbiters, or point measurements from landers or rovers.

We identified fourteen scientific topics in seven broad areas that, in the view of JPL scientists, can \emph{only} be investigated through geographically distributed, spatially and temporally correlated measurements - i.e., the type of measurements that can only be provided by a distributed instrument (Table \ref{tab:sciencecase:ranking}).

From these, we down-selected four scientific topics that are clearly identified as high-priority in Decadal Surveys; are well-aligned with JPL core competencies or (in one case) represent promising areas for future growth; and which could feasibly be addressed with existing and tipping-point technologies:
(a) \textbf{localization of seismic events} on rocky and icy bodies;
(b) \textbf{magnetometry for internal composition} across the Solar System;
(c) \textbf{trace gas detection}, with a focus on Mars; and 
(d) \textbf{global climate and weather} on Mars.


For each of these topics, we outlined its scientific importance according to the Decadal Survey; drafted a high-level distributed instrument architecture; identified critical technological and programmatic challenges that should be addressed; and laid out a preliminary strategy for overcoming these challenges. 

We remark that, in our search, we focused exclusively on the scientific \emph{need} for distributed instruments, i.e., on questions that cannot be addressed with remote sensing or with point measurements. Distributed instruments could also offer additional \emph{engineering benefits} (e.g., faster coverage, lower cost, or higher resilience) compared to a monolithic instrument for other science questions. The investigation of such engineering benefits is beyond the scope of this report, and an interesting direction for future research.

\paragraph{Enabling Technologies}

\begin{displayquote}
\emph{The majority of required technologies are mature and ready for incorporation in a distributed instrument architecture. However, additional focused investments are needed.}
\end{displayquote}

We surveyed the state-of-the-art in enabling technologies for distributed instruments, namely, EDL and sensor placement, localization and synchronization, communications, on-board computation and storage, adaptive sampling and instrument autonomy, power, and thermal control. For each of these technologies, we compared the state-of-the-art with the likely requirements of a distributed instrument architecture for each of the high-priority science topics identified above (Table \ref{tab:enabling-technologies}).

Remarkably, the majority of required technologies are quite mature and ready for incorporation in a distributed instrument architecture. However, further investments are required in three key areas:
\begin{itemize}
\item  \textbf{EDL and sensor placement  techniques} that can ensure global access to planetary surfaces, tailored to specific Solar System bodies of interest;
\item \textbf{Compact and long-lasting power solutions} for sensing units, especially for high latitudes and for exploration of bodies in the outer Solar System; 
\item \textbf{Instrument autonomy}, especially data compression for distributed seismology and active sampling techniques to curtail power requirements for all classes of distributed instruments.
\end{itemize}

JPL is already investing significantly in these areas; these investments should be sustained to ensure that the potential of distributed instruments can be fully realized.

\paragraph{Programmatic Recommendations}

\begin{displayquote}
\emph{
JPL should conduct detailed architecture design studies for distributed instruments, continue funding key technologies, and support Earth analog field campaigns. %
}
\end{displayquote}

Distributed instruments are uniquely well-positioned to address a number of high priority scientific questions, and key technologies are either mature or well on their way to feasibility. To fully realize the promise of distributed instruments, JPL should make strategic investments to:

\textbf{Further develop the architectures of distributed instruments} for high-priority science questions that were drafted in this report through detailed design exercises (e.g., Team-X). These design exercises will validate the feasibility of the current draft architectures, explore and resolve system-level trades, and result in detailed instrument architectures ready for infusion in future mission proposals. 

\textbf{Sustain existing technology investments} in EDL and sensor placement, compact power solutions, and instrument autonomy. Technology gaps in these three areas should be filled before distributed instruments can be proposed as part of future mission architectures.

\textbf{Support Earth analog field tests} for distributed instruments. The benefit of Earth analog field tests is threefold: tests will (a) validate the scientific potentials and technology feasibility of distributed instruments, (b) bring into relief any ``unknown unknowns'' that should be resolved prior to additional development, and, critically, (c) give JPL first-hand experience into the \emph{operations} of distributed instruments, which is likely to be a novel and complex challenge.

In addition to these strategic activities, we also recommend that JPL \emph{foster multidisciplinary collaborations through workshops and seminar series} to accelerate the development of distributed instruments. The design, development, and operation of distributed instruments requires multidisciplinary skills and teams, including not only scientific expertise and know-how in the design of individual detectors, but also expertise in, e.g., communications, localization, time synchronization, and on-board autonomy. On the upside, technology developments in these areas are applicable to many distributed instruments, irrespective of the underlying science question. Accordingly, fostering long-term multidisciplinary collaborations between scientists and technologists is critical to catalyze future distributed instrument designs. Such collaborations could be fostered by creating venues for multidisciplinary collaboration, e.g., a seminar series and a yearly workshop.

